Sparse POD Mode Selection and Manifold Dimensionality Reduction with Neural Networks

Linear dimensionality reduction methods such as proper orthogonal decomposition (POD) make high-dimensional data amenable to analysis by identifying the principal components, or modes, that capture the most variance, or energy, in the data and constructing a low-dimensional representation in the subspace they span. Such linear methods struggle, however, for data with slowly decaying Kolmogorov $n$-widths, such as advection-dominated and turbulent flows, which require many modes for accurate reconstruction; moreover, energy-based truncation can discard low-energy modes needed to capture small-scale features. Recent nonlinear manifold methods using polynomial mappings with alternating or greedy mode selection achieve better reconstruction with fewer modes, but fix the form of the nonlinear mapping a priori, limiting expressivity. In contrast, neural network (NN) manifolds offer greater expressivity yet employ energy-based selection. We present SparseModesNet, a dimensionality reduction framework that employs linear encoding and nonlinear NN decoding. The decoder leverages LassoNet, a method enforcing hierarchical sparsity through a residual connection with a linear skip layer, to simultaneously select informative modes and learn a nonlinear mapping that minimizes reconstruction error. On benchmark advection-dominated and chaotic flows, SparseModesNet matches or exceeds state-of-the-art performance. For turbulent channel flow at friction Reynolds number $Re_\tau = 5200$, our method reduces reconstruction error by 51-78% compared to existing polynomial manifold methods while maintaining interpretability through physically meaningful mode selection.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> sections/supplements/ablation.tex <==
\section{Comparison Study of Different Mode Selection Strategies}\label{sec:sup:ablation}

As discussed in~\Cref{sec:sparsemodesnet:design}, SparseModesNet differs from the original LassoNet framework in that the \gls*{nn} component receives only the selected modes (\( \omegavec \odot \zvec \)) rather than the full candidate set (\( \zvec \)). Following the original LassoNet framework instead would yield the optimization problem
\begin{equation}\label{eqn:ablation:lassonet-style}
    \begin{gathered}
        \min_{\omegavec,\hnn, \Wmat}\sum_{i=1}^n \bigl \lVert \xvec_i - \Umat_s (\omegavec \odot \zvec_i) - \Wmat\hnn(\zvec_i) \bigr \rVert_2^2 + \lambda \| \omegavec \|_1 \\
        \text{subject to} ~~
        \| \Wcal_j^{(1)}\|_\infty \leq M|\omega_j|~~
        \text{and}~~
        {[\Umat_s\diag(\1_{\{\omega_j\neq 0\}}(\omegavec))]}^\top\Wmat= 0, ~\forall j \in [s].
    \end{gathered}
\end{equation}

We also discussed how, when both components receive the same selected-mode input, the hierarchical sparsity constraint may be unnecessary and a simpler \( \ell_1 \) regularization on \( \omegavec \) might suffice, yielding the alternative problem:
\begin{equation}\label{eqn:ablation:l1-only}
    \begin{gathered}
        \min_{\omegavec,\hnn, \Wmat}\sum_{i=1}^n \bigl \lVert \xvec_i - \Umat_s (\omegavec \odot \zvec_i) - \Wmat\hnn(\omegavec \odot \zvec_i) \bigr \rVert_2^2 + \lambda \| \omegavec \|_1 \\
        \text{subject to} \quad 
        {[\Umat_s\diag(\1_{\{\omega_j\neq 0\}}(\omegavec))]}^\top\Wmat= 0, ~\forall j \in [s].
    \end{gathered}
\end{equation}

To evaluate SparseModesNet against these alternatives, we compare three mode selection strategies:
\begin{itemize}
    \item \textbf{SparseModesNet (Proposed)}: as in~\cref{eqn:lassonet-opt}, the \gls*{nn} component receives only the selected modes (\( \omegavec \odot \zvec \)) and the hierarchical sparsity constraint is enforced.
    \item \textbf{LassoNet with \( h_{\mathrm{NN}}(\zvec) \) (unmasked)}: the \gls*{nn} component receives the full candidate set (\( \zvec \)) while the hierarchical sparsity constraint is retained, as in~\cref{eqn:ablation:lassonet-style}.
    \item \textbf{\( \ell_1 \)-penalty only}: the \gls*{nn} component receives only the selected modes (\( \omegavec \odot \zvec \)) but uses only \( \ell_1 \) regularization on \( \omegavec \), without the hierarchical sparsity constraint, as in~\cref{eqn:ablation:l1-only}.
\end{itemize}

We adopt the experimental setup of~\Cref{sec:numerics:pulse}, training a nonlinear decoder for a \( \Pi_2 \)-Net model while selecting modes that minimize the reconstruction error for the linear transport equation. To account for variability due to random initialization of \gls*{nn} weights and biases, we repeat the training 100 times per method and report the statistics of the final reconstruction error at reduced dimension \( r = 15 \), along with the mode selection patterns. For a fair comparison, the stopping criteria and hyperparameters are kept consistent across all three methods, with mode selection stopped once the number of modes decreases to \( r = 15 \).

\Cref{fig:ablation:index_selection} presents the frequency of selecting each POD mode over the 100 runs per method, while~\Cref{fig:ablation:reconstruction_error} shows the corresponding box plots of reconstruction errors. SparseModesNet selects a more diverse range of modes, including lower-energy ones, whereas both the \( \ell_1 \)-penalty only and LassoNet-style variants exhibit a strong bias toward higher-energy modes, commonly known as the \emph{spectral bias}~\cite{rahaman2019spectral}.

\begin{figure}[htpb!]
    \centering
    \includegraphics[width=\textwidth]{figures/ablation/index_selection_frequency.pdf} 
    \vspace{-1em}
    \caption{Comparison of the three different mode selection strategies in terms of the frequency of selecting each POD mode over 100 independent training runs. The proposed SparseModesNet framework (\textbf{left}) selects a wider range of modes including low-energy modes, while the \( \ell_1 \)-penalty only variant (\textbf{middle}) and LassoNet-style variant (\textbf{right}) exhibit a strong bias toward selecting higher-energy modes.}\label{fig:ablation:index_selection}
\end{figure}

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=\textwidth]{figures/ablation/relative_error_boxplot.pdf} 
    \vspace{-1em}
    \caption{Box plot of the reconstruction error for the three different mode selection strategies over 100 independent training runs. The proposed SparseModesNet framework (bottom) achieves significantly lower reconstruction error with substantially less variability compared to the other two variants.}\label{fig:ablation:reconstruction_error}
\end{figure}

Quantitatively, SparseModesNet achieves the lowest mean reconstruction error (\( \mu = 1.81 \times 10^{-8} \)) with minimal variability (\( \sigma = 1.86 \times 10^{-8} \)). The LassoNet-style variant is moderate (\( \mu = 1.33 \times 10^{-7} \), \( \sigma = 1.42 \times 10^{-7} \)), roughly a 7-fold increase over SparseModesNet, while the \( \ell_1 \)-penalty only variant is far worse (\( \mu = 6.04 \times 10^{-6} \), \( \sigma = 3.85 \times 10^{-6} \))---more than 300 times higher than the proposed method. This suggests that the hierarchical sparsity constraint, combined with feeding selected modes to both components, encourages the selection of modes that may not be the most energetic yet yield superior reconstruction.

The \( \ell_1 \)-penalty only variant strongly favors the most energetic modes and rarely selects lower-energy ones. In the rare cases when it does, it attains reconstruction errors comparable to SparseModesNet, as seen in the low-error outliers in~\Cref{fig:ablation:reconstruction_error}, but this behavior is inconsistent and infrequent. The LassoNet-style variant, which enforces the hierarchical sparsity constraint but feeds the full candidate set to the \gls*{nn} component, also biases toward higher-energy modes; this likely drives its higher reconstruction errors relative to SparseModesNet, though it still substantially outperforms the \( \ell_1 \)-penalty only approach. Overall, SparseModesNet consistently identifies relevant modes that yield superior reconstruction compared to the alternatives.

\Cref{fig:ablation:mode_elimination} illustrates the mode elimination process of a single training instance over the entire regularization path, including intermediate epochs for each \( \lambda \). SparseModesNet eliminates modes monotonically, whereas the other two variants spuriously reactivate previously eliminated modes---consistent with our monotonic mode elimination results in~\Cref{sec:sup:monotonic}. We also observe faster sparsification in SparseModesNet than in the LassoNet-style variant, matching the insight from~\Cref{remark:gskip-small} that the network gradient can accelerate the shrinkage of \( \omega_j \) as it becomes less informative.

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/ablation/mode_elimination_bar.pdf} 
    \caption{Comparison of mode elimination for a single training instance throughout the entire regularization path including intermediate epochs for each \(\lambda \) value. Our proposed SparseModesNet shows monotonic mode elimination while the other shows spurious reactivation of previously eliminated modes.}\label{fig:ablation:mode_elimination}
\end{figure}

==> sections/supplements/architecture.tex <==
\section{Hybrid Neural Network Architecture}\label{sec:sup:architecture}

This section details the \gls*{nn} architecture used in SparseModesNet, consisting of a Deep Polynomial \glspl*{nn} known as \( \Pi \)-Nets~\cite{chrysos2022Deep}, and their combination with a linear layer to form the hybrid architecture used in our experiments.

\subsection{Deep Polynomial Neural Networks}\label{sec:sup:architecture:pinets}
Deep Polynomial \glspl*{nn}, or \( \Pi \)-Nets~\cite{chrysos2022Deep}, are function approximators whose output is a high-order polynomial of the input, in contrast to standard Deep Convolutional \glspl*{nn} (DCNNs), which compose linear operators with nonlinear activations.
While any smooth function admits a polynomial approximation, a direct implementation suffers a combinatorial explosion in parameters, growing as \( \mathcal{O}(o^N) \) for an \( o \)-dimensional input and an \( N^{th} \)-order polynomial.
To overcome this, \( \Pi \)-Nets cast parameter estimation as a coupled tensor factorization: decomposing the high-order parameter tensors and enforcing factor sharing sharply reduces the number of learnable parameters and enables an efficient implementation through hierarchical neural network architectures.

A vector-valued function \( g(\yvec):\mathbb{R}^{o}\rightarrow\mathbb{R}^{p} \) (with \( o \) an arbitrary input dimension) is modeled as an \( N^{th} \)-order multivariate polynomial of \( \yvec \), whose vectorized output \( \vvec \) is
\begin{equation}\label{eq:poly_func}
    \vvec =g(\yvec)=\betavec_\pi + \sum_{n=1}^{N}\left(\Wcal^{(n)}_\pi\prod_{j=2}^{n+1}\times_{j}\yvec\right) 
\end{equation}
where \( \betavec_\pi\in\mathbb{R}^{p} \) is a bias term and \( {\{\Wcal^{(n)}_\pi\in\R^{p\times o \times \cdots \times o} \}}_{n=1}^{N} \) are the learnable parameter tensors for each order \( n \). We distinguish the first-layer weight \( \Wcal^{(1)} \) of our SparseModesNet architecture from the \( \Pi \)-Net layer tensors \( \Wcal^{(n)}_\pi \), \( n=1,\ldots,N \).

The core innovation of \( \Pi \)-Nets is structuring these tensors through joint decompositions: all \( \{\Wcal^{(n)}_\pi \}_{n=1}^{N} \) are jointly factorized via a coupled CANDECOMP/PARAFAC (CP) decomposition~\cite{carroll1970analysis,harshman1970foundations}, with factors for lower-order terms shared. Denote the matrix form of the CP decomposition of \( \Wcal^{(n)}_\pi \) by \( \Wmat^{(n)}_\pi \in \R^{p \times o^n} \), and the factor matrices by \( \Cmat \in \R^{p \times k} \) and \( \Pmat_n \in \R^{o \times k} \), \( n=1,\ldots,N \), where \( k \) is the CP rank. For example, a 3\textsuperscript{rd}-order polynomial is
\begin{equation*}
    \begin{aligned}
        g(\yvec) \;=\; &\betavec_\pi + \Cmat\Pmat_{1}^\top\yvec + \Cmat{(\Pmat_{3} * \Pmat_{1})}^\top (\yvec * \yvec) + \Cmat{(\Pmat_{2} * \Pmat_{1})}^\top (\yvec * \yvec)  \\
        & + \Cmat{(\Pmat_{3} * \Pmat_{2} * \Pmat_{1})}^\top (\yvec * \yvec * \yvec)  
    \end{aligned}
\end{equation*}
where \( * \) denotes the Khatri-Rao or column-wise Kronecker product. This polynomial can then be generalized by the following recursive relation:
\begin{equation}\label{eqn:pinet-recursive}
    \vvec_n = (\Pmat_{n}^\top \yvec) \odot \vvec_{n-1} + \vvec_{n-1}, \quad n=2,\ldots,N
\end{equation}
with \( \vvec_1 = \Cmat(\Pmat_{1}^\top \yvec) \) and \( \vvec = \Cmat\vvec_N + \betavec_\pi \), where \( \odot \) is the element-wise product and \( \betavec_\pi \) an optional bias. This recursive form shows how a standard linear or convolutional layer becomes a polynomial one; see~\cite{chrysos2022Deep} for details.
In practice, one defines the polynomial order \( N \) and CP rank \( k \), takes \( \Cmat \), \( \Pmat_{n} \), and \( \betavec_\pi \) as learnable parameters, and computes the forward model via the recursion~\eqref{eqn:pinet-recursive}, enabling efficient training and inference.

\subsection{Hybrid Architecture: Fully Connected Layer + \texorpdfstring{\( \Pi \)-Net}{Pi-Net}}\label{sec:sup:architecture:hybrid}

Although the \( \Pi \)-Net is itself highly expressive through polynomial expansions, a hybrid approach can be beneficial when reconstructing data with both linear and nonlinear characteristics from a limited number of modes. We therefore combine a standard fully connected layer with a \( \Pi \)-Net, leveraging the strengths of both standard \gls*{nn} transformations and polynomial approximations.
\Cref{fig:architecture} shows the schematic. The portion following the first layer realizes the recursion~\cref{eqn:pinet-recursive} for a 3\textsuperscript{rd}-order polynomial, which takes the first-layer output as input in the form:
\begin{equation}
    \yvec = \Wcal^{(1)}(\omegavec\odot\zhat) + \betavec^{(1)} \in \R^o,
\end{equation}
with an identity activation, first-layer weights \( \Wcal^{(1)} \in \R^{o \times s} \), and bias \( \betavec^{(1)} \in \R^o \).
This affine layer maps the input features/modes into a representation better suited for the \( \Pi \)-Net to capture polynomial nonlinearities, and also serves as the gate layer where the hierarchical sparsity constraint is applied during training.

\begin{figure}[htbp!]
    \centering
    {Hybrid Architecture (\( \Pi_3\)-Net): Fully Connected Layer + 3\textsuperscript{rd}-Order \( \Pi \)-Net}
    \includegraphics[width=0.95\textwidth]{figures/hybrid-pi-net-architecture.pdf}
    \vspace{-1.5em}
    \caption{Schematic of the hybrid architecture combining a fully connected layer with a \( \Pi \)-Net. The input first passes through a fully connected layer, which is then fed into the \( \Pi \)-Net to produce the final output. This architecture leverages the strengths of both linear transformations and polynomial approximations for enhanced expressivity.}\label{fig:architecture}
\end{figure}

This choice is necessary because applying the hierarchical sparsity constraint directly to the \( \Pi \)-Net CP factors would be non-trivial and complicate training. Placing it on the fully connected layer lets us control mode selection while retaining the polynomial expressivity of the \( \Pi \)-Net.

We note that this shallow hybrid---a single fully connected layer with no nonlinear activation followed by a \( \Pi \)-Net---performed best in our experiments, outperforming deeper variants with additional fully connected layers before or after the \( \Pi \)-Net. This suggests that complicated architectures are unnecessary for reconstructing data from a limited number of modes, as the \( \Pi \)-Net already provides sufficient expressivity.



==> sections/supplements/theory.tex <==
\section{Theoretical Analysis of SparseModesNet's Design Choice}\label{sec:sup:sparsemodesnet:theory}

We establish theoretical foundations for the design choices in SparseModesNet. 

\subsection{Assumptions \& Constraints}

Throughout this section, we impose the following standing assumptions and constraints.

\begin{assumption}\label[assumption]{ass:data}
    The training data \( \{\xvec_i\}_{i=1}^n \subset \R^d \) as well as projected data \( \{\hat{\zvec}_i\}_{i=1}^n \subset \R^s \) satisfy \( \hat{\zvec}_i \neq \mathbf{0} \) for all \( i \in [n] \).
\end{assumption}

\begin{assumption}\label[assumption]{ass:nn} 
    The \gls{nn} \( \hnn: \R^s \to \R^p \) is continuously differentiable, composed of several affine transformations and smooth activations (e.g., \(\tanh \)). Its Jacobian is denoted \( \Jmat_\hnn(\zetavec) = \partial \hnn / \partial \zetavec \in \R^{p \times s} \).
\end{assumption}

\begin{constraint}\label[constraint]{ass:hier}
    The first-layer weights \( \Wcal^{(1)} \in \R^{p_1 \times s} \) and skip weights \( \omegavec \in \R^s \) satisfy \( \|\Wcal_j^{(1)}\|_\infty \leq M|\omega_j| \) for all \( j \in [s] \), where \( M > 0 \) is the hierarchy coefficient and \( \Wcal_j^{(1)} \in \R^{p_1} \) denotes the \( j \)-th column of \( \Wcal^{(1)} \)~\cite{lemhadri2021Lassonet}.
\end{constraint}

\subsection{Notation}\label{sec:sup:notation}

The standard basis vector in \( \R^s \) with \( 1 \) in position \( j \) is denoted \( \evec_j \). For \( \omegavec \in \R^s \), we define \( \diag(\omegavec) \in \R^{s \times s} \) as the diagonal matrix with entries \( [\diag(\omegavec)]_{jj} = \omega_j \). Note that the elementwise product \( \omegavec \odot \hat{\zvec}_i \) equals \( \diag(\omegavec)\hat{\zvec}_i \). We denote \( \Theta \) to be the collection of \gls{nn} parameters. 

We distinguish two types of superscripts throughout this section:
\begin{itemize}
    \item For a regularization parameter \( \lambda > 0 \), the pair \( (\omegavec^*(\lambda), \Theta^*(\lambda)) \) denotes a  \emph{stationary point} of the regularized objective~\eqref{eqn:regularized_objective}, i.e., a point satisfying the first-order optimality (KKT) conditions for the constrained problem.
    \item Given current values \( (\omega_j, \Wcal_j^{(1)}) \), the notation \( (\omega_j^+, \Wcal_j^{(1)+}) \) denotes the output of a single proximal gradient iteration.
\end{itemize}
For a regularization parameter \( \lambda > 0 \), the \emph{active set} at a stationary point is
\begin{displaymath}
    \Acal(\lambda) = \{j \in [s] : \omega_j^*(\lambda) \neq 0\}.
\end{displaymath}

\subsection{The SparseModesNet Objective}

Define the mean-squared error loss functional \( \Lcal: \R^s \times \Theta \to \R \) by
\begin{equation}\label{eqn:loss_functional}
    \Lcal(\omegavec, \Theta) = \frac{1}{n} \sum_{i=1}^n \bigl\|\xvec_i - \Umat_s \diag(\omegavec) \hat{\zvec}_i - \Wmat \hnn(\diag(\omegavec) \hat{\zvec}_i; \Theta)\bigr\|_2^2.
\end{equation}
The regularized objective subject to the Hierarchical~\Cref{ass:hier} is then
\begin{equation}\label{eqn:regularized_objective}
    \min_{\omegavec, \Theta} \; \Jcal_\lambda(\omegavec, \Theta) := \Lcal(\omegavec, \Theta) + \lambda \|\omegavec\|_1 .
\end{equation}

\subsection{Gradient Structure Analysis}

We first establish the precise form of the gradient and contrast it with the standard LassoNet architecture.

\begin{definition}[Masked vs.\ unmasked architectures]\label{def:architectures}
    \leavevmode
    \begin{itemize}
        \item The \emph{masked architecture} (SparseModesNet) uses the \gls{nn} input that masks \( \hat{\zvec}_i \) with the mode selector weight \( \omegavec \), i.e., \( \zetavec_i(\omegavec) = \diag(\omegavec) \hat{\zvec}_i \in \R^s \).
        \item The \emph{unmasked architecture} (standard LassoNet, cf.~\Cref{remark:why-lassonet-unmask}) uses the \gls{nn} input \( \zetavec_i = \hat{\zvec}_i \in \R^s \), independent of \( \omegavec \).
    \end{itemize}
\end{definition}

\begin{definition}\label{def:residual}
    Define the residual vector \( \rvec_i(\omegavec, \Theta) \in \R^d \) by
    \begin{equation}\label{eqn:residual}
        \rvec_i(\omegavec, \Theta) = \xvec_i - \Umat_s \diag(\omegavec) \hat{\zvec}_i - \Wmat \hnn(\diag(\omegavec) \hat{\zvec}_i; \Theta).
    \end{equation}
    Then, the loss functional admits the representation
    \begin{displaymath}
        \Lcal(\omegavec, \Theta) = \frac{1}{n} \sum_{i=1}^n \|\rvec_i(\omegavec, \Theta)\|_2^2
    \end{displaymath}
    and is continuously differentiable in \( (\omegavec, \Theta) \).
\end{definition}
The loss representation is immediate from~\Cref{def:residual} and its continuous differentiability follows from~\Cref{ass:nn} and the chain rule, noting that \( \diag(\omegavec) \hat{\zvec}_i \) is linear in \( \omegavec \) and \( \hnn \) is \( C^1 \) by assumption.

\begin{lemma}\label[lemma]{lem:gradient_sparsemodesnet}
    Under~\Cref{ass:data,ass:nn}, the gradient of the loss functional with respect to \( \omega_j \) for \( j \in [s] \) is
    \begin{equation}\label{eqn:gradient_compact}
        \frac{\partial \Lcal}{\partial \omega_j} = -\frac{2}{n}\sum_{i=1}^n \hat{z}_{ij} \cdot \rvec_i^\top \bigl[\uvec_j + \Wmat \Jmat_\hnn(\diag(\omegavec) \hat{\zvec}_i) \evec_j\bigr],
    \end{equation}
    where \( \uvec_j \in \R^d \) is the \( j \)-th column of \( \Umat_s \), \( \hat{z}_{ij} = [\hat{\zvec}_i]_j \) is the \( j \)-th component of \( \hat{\zvec}_i \), and \( \Jmat_\hnn(\cdot) \in \R^{p \times s} \) is the Jacobian of \( \hnn \).
\end{lemma}

\begin{proof}
    Fix \( j \in [s] \). Differentiating under the sum:
    \begin{displaymath}
        \frac{\partial \Lcal}{\partial \omega_j} = \frac{1}{n} \sum_{i=1}^n \frac{\partial}{\partial \omega_j} \|\rvec_i\|_2^2 = \frac{2}{n}\sum_{i=1}^n \rvec_i^\top \frac{\partial \rvec_i}{\partial \omega_j}.
    \end{displaymath}
    We compute \( \partial \rvec_i / \partial \omega_j \) term by term.
    
    \textbf{Term 1: Linear skip connection.} Since \( [\diag(\omegavec) \hat{\zvec}_i]_k = \omega_k \hat{z}_{ik} \), we have \( \partial[\diag(\omegavec) \hat{\zvec}_i]_k / \partial \omega_j = \delta_{jk} \hat{z}_{ik} = \hat{z}_{ij} \delta_{jk}\), giving \( \partial[\diag(\omegavec) \hat{\zvec}_i] / \partial \omega_j = \hat{z}_{ij} \evec_j \). Therefore,
    \begin{displaymath}
        \frac{\partial}{\partial \omega_j} \bigl[\Umat_s \diag(\omegavec) \hat{\zvec}_i\bigr] = \hat{z}_{ij} \Umat_s \evec_j = \hat{z}_{ij} \uvec_j.
    \end{displaymath}
    
    \textbf{Term 2: \Gls{nn} branch.} Define \( \zetavec_i = \diag(\omegavec) \hat{\zvec}_i \). By the chain rule:
    \begin{displaymath}
        \frac{\partial}{\partial \omega_j} \bigl[\Wmat \hnn(\zetavec_i)\bigr] = \Wmat \Jmat_\hnn(\zetavec_i) \frac{\partial \zetavec_i}{\partial \omega_j} = \hat{z}_{ij} \Wmat \Jmat_\hnn(\zetavec_i) \evec_j.
    \end{displaymath}
    
    \textbf{Combining terms:} Since \( \rvec_i = \xvec_i - \Umat_s \diag(\omegavec) \hat{\zvec}_i - \Wmat \hnn(\zetavec_i) \),
    \begin{displaymath}
        \frac{\partial \rvec_i}{\partial \omega_j} = -\hat{z}_{ij} \bigl[\uvec_j + \Wmat \Jmat_\hnn(\diag(\omegavec) \hat{\zvec}_i) \evec_j\bigr].
    \end{displaymath}
    Substituting yields~\eqref{eqn:gradient_compact}.
\end{proof}


\begin{lemma}\label[lemma]{lem:gradient_lassonet}
    In the unmasked architecture (\Cref{def:architectures}) where the \gls{nn} input is \( \hat{\zvec}_i \), the gradient of the loss with respect to \( \omega_j \) reduces to
    \begin{equation}\label{eqn:gradient_lassonet_only}
        \frac{\partial \Lcal}{\partial \omega_j} = -\frac{2}{n}\sum_{i=1}^n \hat{z}_{ij} \cdot \rvec_i^\top \uvec_j.
    \end{equation}
\end{lemma}

\begin{proof}
    In the unmasked case, the \gls{nn} term \( \Wmat \hnn(\hat{\zvec}_i; \Theta) \) is independent of \( \omegavec \), so \( \frac{\partial}{\partial \omega_j} [\Wmat \hnn(\hat{\zvec}_i; \Theta)] = \mathbf{0} \). The result follows from Term~1 of the proof of~\Cref{lem:gradient_sparsemodesnet}.
\end{proof}

\begin{definition}\label{def:gradient_coupling}
    Define the \emph{skip gradient} and \emph{network gradient} components:
    \begin{align}
        G_j^{\mathrm{skip}}(\omegavec, \Theta) &= -\frac{2}{n}\sum_{i=1}^n \hat{z}_{ij} \cdot \rvec_i(\omegavec, \Theta)^\top \uvec_j, \label{eqn:Gskip} \\
        G_j^{\mathrm{net}}(\omegavec, \Theta) &= -\frac{2}{n}\sum_{i=1}^n \hat{z}_{ij} \cdot \rvec_i(\omegavec, \Theta)^\top \Wmat \Jmat_\hnn(\diag(\omegavec) \hat{\zvec}_i) \evec_j. \label{eqn:Gnet}
    \end{align}
    Then for SparseModesNet: \( \partial \Lcal / \partial \omega_j = G_j^{\mathrm{skip}} + G_j^{\mathrm{net}} \), while for standard LassoNet: \( \partial \Lcal / \partial \omega_j = G_j^{\mathrm{skip}} \).
\end{definition}

\begin{remark}\label[remark]{remark:gskip-small}
    As training progresses and mode \( j \) becomes less informative, the residuals \( \rvec_i \) are increasingly explained by the remaining active modes or by those beyond the \( s \) candidates, causing \( \rvec_i \) to lie approximately orthogonal to \( \uvec_j \), and hence drives \( |G_j^{\mathrm{skip}}| \) toward zero. Consequently, the network gradient \( G_j^{\mathrm{net}} \) in~\eqref{eqn:Gnet} can dominate the overall gradient in SparseModesNet, accelerating the shrinkage of \( \omega_j \).
\end{remark}

\subsection{Proof of Monotonic Mode Elimination}\label{sec:sup:monotonic}

We now prove the monotonic mode elimination property stated in~\Cref{sec:sparsemodesnet:design} of the main text. We begin by establishing lemmas on the nullification of weights and gradients induced by the hierarchical constraint and input masking.

\subsubsection{Preliminary Lemmas}

\begin{lemma}[Constraint-induced weight nullification]\label{lem:weight_null}
    Under the Hierarchical~\Cref{ass:hier}, if \( \omega_j = 0 \) for some \( j \in [s] \), then \( \Wcal_j^{(1)} = \mathbf{0} \in \R^{p_1} \).
\end{lemma}

\begin{proof}
    The constraint \( \|\Wcal_j^{(1)}\|_\infty \leq M|\omega_j| = 0 \) implies \( |[\Wcal_j^{(1)}]_k| \leq 0 \) for all \( k \in [p_1] \). Since \( |\cdot| \geq 0 \), we have \( [\Wcal_j^{(1)}]_k = 0 \) for all \( k \), i.e., \( \Wcal_j^{(1)} = \mathbf{0} \).
\end{proof}

\begin{lemma}[Input nullification]\label{lem:input_null}
    If \( \omega_j = 0 \), then the \( j \)-th component of the masked input vanishes: \( [\diag(\omegavec) \hat{\zvec}_i]_j = 0 \) for all \( i \in [n] \).
\end{lemma}

\begin{proof}
    Direct computation: \( [\diag(\omegavec) \hat{\zvec}_i]_j = \omega_j \hat{z}_{ij} = 0 \).
\end{proof}

\begin{lemma}[Gradient severance]\label[lemma]{lem:gradient_severance}
    Suppose \( \omega_j = 0 \) for some \( j \in [s] \). Under the masked architecture (\Cref{def:architectures}), the gradient of the loss \( \Lcal \) with respect to the first-layer weights \( \Wcal_j^{(1)} \) satisfies
    \begin{displaymath}
        \frac{\partial \Lcal}{\partial \Wcal_j^{(1)}} = \mathbf{0} \in \R^{p_1}.
    \end{displaymath}
\end{lemma}

\begin{proof}
    Let the \gls{nn} have the form \( \hnn(\zetavec; \Theta) = \hnn^{(L)} \circ \cdots \circ \hnn^{(2)} \circ \hnn^{(1)}(\zetavec) \), where \( \hnn^{(1)}(\zetavec) = \sigma(\Wcal^{(1)}\zetavec + \betavec^{(1)}) \) with elementwise activation \( \sigma \). Define the preactivation \( \avec^{(1)}(\zetavec) = \Wcal^{(1)}\zetavec + \betavec^{(1)} \in \R^{p_1} \).
    
    For the masked input \( \zetavec_i = \diag(\omegavec) \hat{\zvec}_i \), the \( k \)-th component of the preactivation is
    \begin{displaymath}
        [\avec^{(1)}(\zetavec_i)]_k = \sum_{m=1}^s [\Wcal^{(1)}_m]_{k} \omega_m \hat{z}_{im} + [\betavec^{(1)}]_k.
    \end{displaymath}
    Differentiating with respect to \( [\Wcal_j^{(1)}]_k \) (the \( (k,j) \)-entry of \( \Wcal^{(1)} \)):
    \begin{displaymath}
        \frac{\partial [\avec^{(1)}(\zetavec_i)]_k}{\partial [\Wcal_j^{(1)}]_k} = \omega_j \hat{z}_{ij}.
    \end{displaymath}
    
    By the chain rule:
    \begin{displaymath}
        \frac{\partial \Lcal}{\partial \Wcal_j^{(1)}} = \frac{2}{n}\sum_{i=1}^n \frac{\partial \Lcal}{\partial \avec^{(1)}(\zetavec_i)} \cdot \frac{\partial \avec^{(1)}(\zetavec_i)}{\partial \Wcal_j^{(1)}} = \frac{2}{n}\sum_{i=1}^n \omega_j \hat{z}_{ij} \cdot \frac{\partial \Lcal}{\partial \avec^{(1)}(\zetavec_i)}.
    \end{displaymath}
    When \( \omega_j = 0 \), \( \frac{\partial \Lcal}{\partial \Wcal_j^{(1)}} = \mathbf{0} \) regardless of the values of \( \hat{z}_{ij} \) and \( \partial \Lcal / \partial \avec^{(1)}(\zetavec_i) \).
\end{proof}

\begin{remark}\label{remark:gradient_severance_interpretation}
    \Cref{lem:gradient_severance} shows that input masking causes the gradient with respect to \( \Wcal_j^{(1)} \) to vanish when \( \omega_j = 0 \). This severs mode \( j \): no gradient signal can update \( \Wcal_j^{(1)} \). In the unmasked architecture, by contrast, \( \partial \Lcal / \partial \Wcal_j^{(1)} \) is generically nonzero even when \( \omega_j = 0 \), since the \gls{nn} receives the full input \( \hat{\zvec}_i \). However, gradient severance alone only \emph{freezes} \( \Wcal_j^{(1)} \) at its current value; it does not force \( \Wcal_j^{(1)} = \mathbf{0} \). The hierarchical constraint (\Cref{lem:weight_null}) is necessary to ensure that when \( \omega_j = 0 \), the constraint enforces \( \Wcal_j^{(1)} = \mathbf{0} \).
\end{remark}

\subsubsection{The Hier-Prox Operator}

The optimization problem~\eqref{eqn:regularized_objective} is solved via the continuation strategy described in~\Cref{sec:bg:lassonet}, using the hierarchical proximal (Hier-Prox) operator developed in~\cite{lemhadri2021Lassonet}.

\begin{definition}\label{def:pre_proximal}
    In a proximal gradient iteration with step size \( \alpha > 0 \), given current values \( (\omega_j, \Wcal_j^{(1)}) \), the \emph{preproximal values} are
    \begin{equation}\label{eqn:pre_proximal}
        \ot{\omega}_j = \omega_j - \alpha \frac{\partial \Lcal}{\partial \omega_j}, \qquad \ot{\Wcal}_j^{(1)} = \Wcal_j^{(1)} - \alpha \frac{\partial \Lcal}{\partial \Wcal_j^{(1)}}.
    \end{equation}
\end{definition}

\begin{definition}[Hier-Prox operator]\label{def:hierprox}
    For mode \( j \in [s] \), step size \( \alpha > 0 \), regularization parameter \( \lambda > 0 \), hierarchy coefficient \( M > 0 \), and preproximal values \( (\ot{\omega}_j, \ot{\Wcal}_j^{(1)}) \in \R \times \R^{p_1} \), the Hier-Prox operator is
    \begin{equation}\label{eqn:hierprox}
        \mathrm{HierProx}_{\alpha\lambda, M}\bigl(\ot{\omega}_j, \ot{\Wcal}_j^{(1)}\bigr) := \argmin_{(\omega_j, \wvec) \in \Ccal} \; \frac{1}{2}(\omega_j - \ot{\omega}_j)^2 + \frac{1}{2}\|\wvec - \ot{\Wcal}_j^{(1)}\|_2^2 + \alpha\lambda|\omega_j|,
    \end{equation}
    where the constraint set is \( \Ccal = \{(\omega_j, \wvec) \in \R \times \R^{p_1} : \|\wvec\|_\infty \leq M|\omega_j|\} \).
\end{definition}

The constraint set \( \Ccal \) is a double cone with apex at the origin. The Hier-Prox operator produces the updated values \( (\omega_j^+, \Wcal_j^{(1)+}) = \mathrm{HierProx}_{\alpha\lambda, M}(\ot{\omega}_j, \ot{\Wcal}_j^{(1)}) \).

\begin{proposition}[Zero attractor condition]\label{prop:hierprox_zero}
    The Hier-Prox operator satisfies \( \mathrm{HierProx}_{\alpha\lambda, M}(\ot{\omega}_j, \ot{\Wcal}_j^{(1)}) = (0, \mathbf{0}) \) if and only if
    \begin{equation}\label{eqn:hierprox_threshold}
        |\ot{\omega}_j| + M\|\ot{\Wcal}_j^{(1)}\|_1 \leq \alpha\lambda.
    \end{equation}
\end{proposition}

\begin{proof}
    Define \( f(\omega_j, \wvec) = \frac{1}{2}(\omega_j - \ot{\omega}_j)^2 + \frac{1}{2}\|\wvec - \ot{\Wcal}_j^{(1)}\|_2^2 + \alpha\lambda|\omega_j| \). For brevity, write \( \ot{\omega} = \ot{\omega}_j \) and \( \ot{\wvec} = \ot{\Wcal}_j^{(1)} \).
    
    Since \( \Ccal \) is a cone, its tangent cone at the origin equals itself:
    \begin{displaymath}
        T_\Ccal(0, \mathbf{0}) = \Ccal = \bigl\{(d_\omega, \dvec) \in \R \times \R^{p_1} : \|\dvec\|_\infty \leq M|d_\omega|\bigr\}.
    \end{displaymath}
    
    For any direction \( (d_\omega, \dvec) \in T_\Ccal(0, \mathbf{0}) \), the directional derivative of \( f \) at \( (0, \mathbf{0}) \) is
    \begin{displaymath}
        f'((0, \mathbf{0}); (d_\omega, \dvec)) = \lim_{t \to 0^+} \frac{f(t d_\omega, t\dvec) - f(0, \mathbf{0})}{t}.
    \end{displaymath}
    Expanding \( f(t d_\omega, t\dvec) \):
    \begin{displaymath}
    \begin{aligned}
        f(t d_\omega, t\dvec) &= \frac{1}{2}(t d_\omega - \ot{\omega})^2 + \frac{1}{2}\|t\dvec - \ot{\wvec}\|_2^2 + \alpha\lambda|t d_\omega| \\
        &= \frac{1}{2}\ot{\omega}^2 + \frac{1}{2}\|\ot{\wvec}\|_2^2 - t d_\omega \ot{\omega} - t\dvec^\top \ot{\wvec} + \alpha\lambda t|d_\omega| + O(t^2).
    \end{aligned}
    \end{displaymath}
    Since \( f(0, \mathbf{0}) = \frac{1}{2}\ot{\omega}^2 + \frac{1}{2}\|\ot{\wvec}\|_2^2 \), we obtain
    \begin{equation}\label{eqn:directional_derivative}
        f'((0, \mathbf{0}); (d_\omega, \dvec)) = -d_\omega \ot{\omega} - \dvec^\top \ot{\wvec} + \alpha\lambda|d_\omega|.
    \end{equation}
    
    Following the first-order optimality conditions, since \( f \) and a single cone of \( \Ccal \) with the apex at the origin are convex, \( (0, \mathbf{0}) \) is optimal if and only if \( f'((0, \mathbf{0}); (d_\omega, \dvec)) \geq 0 \) for all \( (d_\omega, \dvec) \in T_\Ccal(0, \mathbf{0}) \). We analyze three cases.
    
    \emph{Case 1: \( d_\omega = 0 \).} The constraint forces \( \dvec = \mathbf{0} \), giving \( f'((0, \mathbf{0}); (0, \mathbf{0})) = 0 \geq 0 \).
    
    \emph{Case 2: \( d_\omega > 0 \).} The directional derivative~\eqref{eqn:directional_derivative} becomes \( f'((0, \mathbf{0}); (d_\omega, \dvec)) = d_\omega(\alpha\lambda - \ot{\omega}) - \dvec^\top \ot{\wvec} \). Maximizing \( \dvec^\top \ot{\wvec} \) over \( \|\dvec \|_\infty \leq M d_\omega \) is achieved at \( d_k = M d_\omega \cdot \sign(\ot{w}_k) \) for each coordinate \( k \) where \( \ot{w}_k = {[\ot\wvec]}_k \), yielding
    \begin{displaymath}
        \max_{\|\dvec \|_\infty \leq M d_\omega} \dvec^\top \ot{\wvec} = \sum_{k=1}^{p_1} Md_\omega|\ot{w}_k| = M d_\omega \|\ot{\wvec}\|_1.
    \end{displaymath}
    Thus, the infimum of the directional derivative over \( d_\omega > 0 \) and feasible \( \dvec \) is
    \begin{displaymath}
        \inf_{\substack{d_\omega > 0,\, \|\dvec \|_\infty \leq M d_\omega}} f'((0, \mathbf{0}); (d_\omega, \dvec)) = d_\omega\bigl(\alpha\lambda - \ot{\omega} - M\|\ot{\wvec}\|_1\bigr).
    \end{displaymath}
    For this to be nonnegative for all \( d_\omega > 0 \), we require
    \begin{equation}\label{eqn:case2_condition}
        \ot{\omega} + M\|\ot{\wvec}\|_1 \leq \alpha\lambda.
    \end{equation}
    
    \emph{Case 3: \( d_\omega < 0 \).} Writing \( d_\omega = -\delta \) with \( \delta > 0 \), a similar argument yields
    \begin{equation}\label{eqn:case3_condition}
        -\ot{\omega} + M\|\ot{\wvec}\|_1 \leq \alpha\lambda.
    \end{equation}
    Combining~\eqref{eqn:case2_condition} and~\eqref{eqn:case3_condition} gives \( |\ot{\omega}| + M\|\ot{\wvec}\|_1 \leq \alpha\lambda \), which is~\eqref{eqn:hierprox_threshold}.
\end{proof}

\subsubsection{The Jacobian Structure}

The following fact establishes how the network Jacobian depends on the first-layer weights.

\begin{fact}\label{fact:jacobian_column}
    Consider a \gls{nn} with first layer \( \hnn^{(1)}(\zetavec) = \sigma(\Wcal^{(1)}\zetavec + \betavec^{(1)}) \), where \( \sigma \) is an elementwise activation with derivative \( \sigma' \). Let \( \Jmat^{(L:2)} \) denote the Jacobian of the composition of layers \( 2 \) through \( L \). Then the \( j \)-th column of the network Jacobian satisfies
    \begin{equation}\label{eqn:jacobian_column}
        \Jmat_\hnn(\zetavec) \evec_j = \Jmat^{(L:2)} \cdot \diag\bigl(\sigma'(\Wcal^{(1)}\zetavec + \betavec^{(1)})\bigr) \cdot \Wcal_j^{(1)}.
    \end{equation}
    In particular, if \( \Wcal_j^{(1)} = \mathbf{0} \), then \( \Jmat_\hnn(\zetavec)\evec_j = \mathbf{0} \); and if \( \Wcal_j^{(1)} \neq \mathbf{0} \), then generically \( \Jmat_\hnn(\zetavec)\evec_j \neq \mathbf{0} \).
\end{fact} 

By the chain rule, \( \Jmat_\hnn(\zetavec) = \Jmat^{(L:2)} \cdot \diag(\sigma'(\Wcal^{(1)}\zetavec + \betavec^{(1)})) \cdot \Wcal^{(1)} \). The \( j \)-th column is obtained by right-multiplying by \( \evec_j \), which extracts \( \Wcal_j^{(1)} \). This fact follows from the linearity of this expression in \( \Wcal_j^{(1)} \).

\subsubsection{Additional Assumptions for Monotonicity}

To establish monotonic mode elimination, we impose two regularity conditions on the solution path. These assumptions involve the stationary points \( (\omegavec^*(\lambda), \Theta^*(\lambda)) \) of the regularized objective~\eqref{eqn:regularized_objective} at parameter \( \lambda \).

\begin{assumption}[Lipschitz regularity of the skip gradient]\label[assumption]{ass:lipschitz}
    There exists a constant \( L > 0 \) such that for all regularization parameters \( \lambda, \lambda' \) along the path and all eliminated modes \( j \in [s] \setminus \Acal(\lambda) \cap [s] \setminus \Acal(\lambda') \):
    \begin{displaymath}
        \bigl|G_j^{\mathrm{skip}}(\omegavec^*(\lambda'), \Theta^*(\lambda')) - G_j^{\mathrm{skip}}(\omegavec^*(\lambda), \Theta^*(\lambda))\bigr| \leq L|\lambda' - \lambda|,
    \end{displaymath}
    where \( G_j^{\mathrm{skip}} \) is defined in~\eqref{eqn:Gskip} and \( (\omegavec^*(\lambda), \Theta^*(\lambda)) \) denotes a stationary point of~\eqref{eqn:regularized_objective} at parameter \( \lambda \).
\end{assumption}

\begin{assumption}[Strict complementarity with margin]\label[assumption]{ass:margin}
    There exists a margin \( \delta \in (0, 1) \) such that at each stationary point \( (\omegavec^*(\lambda), \Theta^*(\lambda)) \) of~\eqref{eqn:regularized_objective}, for all eliminated modes \( j \in [s] \setminus \Acal(\lambda) \):
    \begin{displaymath}
        |G_j^{\mathrm{skip}}(\omegavec^*(\lambda), \Theta^*(\lambda))| \leq (1 - \delta)\lambda.
    \end{displaymath}
\end{assumption}

\Cref{ass:lipschitz} requires the skip gradient for eliminated modes to vary Lipschitz-continuously along the solution path. For eliminated modes \( j \), we obtain \( \omega_j^*(\lambda) = 0 \), so \( G_j^{\mathrm{skip}} \) varies only through changes in the residual induced by the active parameters; this dependence is typically well-behaved. \Cref{ass:margin} posits a strict gap between the gradient magnitude \( |G_j^{\mathrm{skip}}| \) and the threshold \( \lambda \). Recalling~\Cref{remark:gskip-small}, \( |G_j^{\mathrm{skip}}| \) is small given \( G_j^{\mathrm{skip}} \) is a weighted sum of inner products \( \rvec_i^\top \uvec_j \) (cf.~\eqref{eqn:Gskip}) with \( \rvec_i \) and \( \uvec_j \) being  nearly orthogonal. The margin \( \delta \) quantifies this gap as a fraction of \( \lambda \), ensuring it grows with the regularization strength.

\subsubsection{Main Result}

\begin{theorem}[Monotonic mode elimination]\label{thm:sup:monotonic}
    Let~\Cref{ass:data,ass:nn,ass:hier,ass:lipschitz,ass:margin} hold. Consider the regularization path \( \lambda_{k+1} = (1 + \epsilon)\lambda_k \) for \( k = 0, 1, \ldots, K-1 \) with path multiplier \( \epsilon > 0 \). Under the SparseModesNet architecture (input masking + hierarchical constraint) optimizing objective~\eqref{eqn:regularized_objective}, if mode \( j \) is eliminated at \( \lambda_k \), i.e., \( \omega_j^*(\lambda_k) = 0 \), then
    \begin{displaymath}
        \omega_j^*(\lambda_\ell) = 0 \quad \text{for all} \quad \ell \geq k,
    \end{displaymath}
    provided one of the following conditions holds:
    \begin{enumerate}
        \item \( L \leq 1 \) and \( \epsilon > 0 \) is arbitrary, or
        \item \( L > 1 \) and  \( 0 < \epsilon \leq \frac{\delta}{L - 1} \),
    \end{enumerate}
    where \( L \) and \( \delta \) are from Assumptions~\ref{ass:lipschitz} and~\ref{ass:margin}, respectively. Equivalently, the active sets are nested: \( \lambda' > \lambda \implies \Acal(\lambda') \subseteq \Acal(\lambda) \).
\end{theorem}

\begin{proof}
    Suppose \( \omega_j^*(\lambda_k) = 0 \) for some mode \( j \) and index \( k \). We show \( \omega_j^*(\lambda_{k+1}) = 0 \); the full result follows by induction.
    
    By~\Cref{lem:weight_null}, the hierarchical constraint forces \( \Wcal_j^{(1)*}(\lambda_k) = \mathbf{0} \). At \( \lambda_{k+1} \), warm-start initialization sets \( (\omega_j, \Wcal_j^{(1)}) = (0, \mathbf{0}) \).
    
    Consider a proximal gradient iteration with step size \( \alpha > 0 \). From~\Cref{def:pre_proximal}, the preproximal values starting from \( (0, \mathbf{0}) \) are
    \begin{displaymath}
        \ot{\omega}_j = 0 - \alpha \frac{\partial \Lcal}{\partial \omega_j}\Big|_{(\omega_j, \Wcal_j^{(1)}) = (0, \mathbf{0})}, \qquad
        \ot{\Wcal}_j^{(1)} = \mathbf{0} - \alpha \frac{\partial \Lcal}{\partial \Wcal_j^{(1)}}\Big|_{(\omega_j, \Wcal_j^{(1)}) = (0, \mathbf{0})}.       
    \end{displaymath}
    By~\Cref{lem:gradient_severance}, \( \frac{\partial \Lcal}{\partial \Wcal_j^{(1)}}\big|_{\omega_j=0} = \mathbf{0} \), hence \( \ot{\Wcal}_j^{(1)} = \mathbf{0} \).
    
    Then, from~\Cref{prop:hierprox_zero}, the zero attractor condition becomes
    \begin{displaymath}
        |\ot{\omega}_j| + M \cdot 0 = \alpha\left|\frac{\partial \Lcal}{\partial \omega_j}\Big|_{(\omega_j, \Wcal_j^{(1)}) = (0, \mathbf{0})}\right| \leq \alpha\lambda_{k+1}.
    \end{displaymath}
    Since \( \omega_j = 0 \) and \( \Wcal_j^{(1)} = \mathbf{0} \), by~\Cref{fact:jacobian_column} we have \( \Jmat_\hnn(\zetavec)\evec_j = \mathbf{0} \), hence \( G_j^{\mathrm{net}} = 0 \) by~\eqref{eqn:Gnet}. The condition simplifies to
    \begin{displaymath}\label{eqn:threshold_simplified}
        |G_j^{\mathrm{skip}}(\omegavec, \Theta)| \leq \lambda_{k+1}.
    \end{displaymath}
    
    By~\Cref{ass:margin}, at the stationary point for \( \lambda_k \):
    \begin{displaymath}
        |G_j^{\mathrm{skip}}(\omegavec^*(\lambda_k), \Theta^*(\lambda_k))| \leq (1 - \delta)\lambda_k.
    \end{displaymath}
    By~\Cref{ass:lipschitz}, at the stationary point for \( \lambda_{k+1} \):
    \begin{displaymath}
    \begin{aligned}
        |G_j^{\mathrm{skip}}(\omegavec^*(\lambda_{k+1}), \Theta^*(\lambda_{k+1}))| &\leq |G_j^{\mathrm{skip}}(\omegavec^*(\lambda_k), \Theta^*(\lambda_k))| + L|\lambda_{k+1} - \lambda_k| \\
        &\leq (1 - \delta)\lambda_k + L\epsilon\lambda_k = \lambda_k(1 - \delta + L\epsilon).
    \end{aligned}
    \end{displaymath}
    For~\eqref{eqn:threshold_simplified} to hold, we need \( \lambda_k(1 - \delta + L\epsilon) \leq \lambda_{k+1} = (1 + \epsilon)\lambda_k \), i.e.,
    \begin{displaymath}
        0 < 1 - \delta + L\epsilon \leq 1 + \epsilon \quad \Longleftrightarrow \quad (L - 1)\epsilon \leq \delta.
    \end{displaymath}
    
    \emph{Case \( L \leq 1 \)}: For any \( \epsilon > 0 \), \( (L-1)\epsilon \leq 0 < \delta \), so the inequality holds.
    
    \emph{Case \( L > 1 \)}: The inequality holds if and only if \( \epsilon \leq \delta/(L-1) \).

    Under the stated conditions, the Hier-Prox operator returns \( (\omega_j^+, \Wcal_j^{(1)+}) = (0, \mathbf{0}) \) at each iteration. The algorithm converges to a stationary point with \( \omega_j^*(\lambda_{k+1}) = 0 \). By~\Cref{ass:margin}, this new stationary point satisfies \( |G_j^{\mathrm{skip}}| \leq (1-\delta)\lambda_{k+1} \), so the argument repeats for subsequent \( \lambda_\ell \), and thus, completing the induction.
\end{proof}

% \begin{remark}\label{remark:severance_role}
%     It is critical that gradient severance (\Cref{lem:gradient_severance}) ensures \( \ot{\Wcal}_j^{(1)} = \mathbf{0} \), eliminating the term \( M\|\ot{\Wcal}_j^{(1)}\|_1 \) from the threshold~\eqref{eqn:hierprox_threshold}. This reduces the Hier-Prox condition to a bound on \( |G_j^{\mathrm{skip}}| \) alone.
% \end{remark}

\begin{remark}[Interpretation of the step size bound]\label{remark:epsilon_interpretation}
    When \( L > 1 \), the bound \( \epsilon \leq \delta/(L-1) \) balances two effects:
    \begin{itemize}
        \item The margin \( \delta \) measures how far below \( \lambda_k \) the gradient \( |G_j^{\mathrm{skip}}| \) lies. Larger \( \delta \) permits larger steps.
        \item The Lipschitz constant \( L \) measures how rapidly \( G_j^{\mathrm{skip}} \) can change. Larger \( L \) requires smaller steps.
    \end{itemize}
    When \( L \leq 1 \), the gradient changes more slowly than the threshold of the zero attractor condition grows, so any path multiplier \( \epsilon \) suffices.
\end{remark}

\subsection{Failure of Monotonicity Without Both Design Choices}\label{sec:sup:failure}

We now show that both input masking and the hierarchical constraint are essential and neither alone guarantees monotonic mode elimination.

\subsubsection{Failure Without Input Masking}

\begin{corollary}\label{cor:reactivation}
    In the unmasked architecture (\Cref{def:architectures}) with the Hierarchical~\Cref{ass:hier} and~\Cref{ass:lipschitz,ass:margin}, there exist problem instances where a mode \( j \), eliminated at \( \lambda_k \), is reactivated at \( \lambda_{k+1} = (1 + \epsilon)\lambda_k \) for any \( \epsilon > 0 \).
\end{corollary}

\begin{proof}
    By~\Cref{lem:weight_null}, warm-start initialization sets \( (\omega_j, \Wcal_j^{(1)}) = (0, \mathbf{0}) \) at \( \lambda_{k+1} \). The preproximal values after one gradient step are
    \begin{displaymath}
        \ot{\omega}_j = -\alpha \frac{\partial \Lcal}{\partial \omega_j}\Big|_{(\omega_j, \Wcal_j^{(1)}) = (0, \mathbf{0})}, \qquad \ot{\Wcal}_j^{(1)} = -\alpha \frac{\partial \Lcal}{\partial \Wcal_j^{(1)}}\Big|_{(\omega_j, \Wcal_j^{(1)}) = (0, \mathbf{0})}.
    \end{displaymath}
    
    In the unmasked architecture, the \gls{nn} input is \( \hat{\zvec}_i \) rather than \( \diag(\omegavec)\hat{\zvec}_i \). The gradient with respect to \( \Wcal_j^{(1)} \) becomes
    \begin{displaymath}
        \frac{\partial \Lcal}{\partial \Wcal_j^{(1)}}\Big|_{(\omega_j, \Wcal_j^{(1)}) = (0, \mathbf{0})} = \frac{2}{n}\sum_{i=1}^n \hat{z}_{ij} \cdot \frac{\partial \Lcal}{\partial \avec^{(1)}(\hat{\zvec}_i)},
    \end{displaymath}
    which is generically \emph{nonzero} since the \gls{nn} observes the full input \( \hat{\zvec}_i \). Hence \( \ot{\Wcal}_j^{(1)} \neq \mathbf{0} \).
    
    By~\Cref{prop:hierprox_zero}, the Hier-Prox operator returns \( (0, \mathbf{0}) \) only if
    \begin{displaymath}
        \left|\frac{\partial \Lcal}{\partial \omega_j}\right| + M\left\|\frac{\partial \Lcal}{\partial \Wcal_j^{(1)}}\right\|_1 \leq \lambda_{k+1}.
    \end{displaymath}
    By~\Cref{ass:margin}, \( |\partial \Lcal / \partial \omega_j| \leq (1-\delta)\lambda_k \) since \( \partial \Lcal / \partial \omega_j = G_{j}^{\mathrm{skip}} \) from~\Cref{def:gradient_coupling}. However, there is no bound on \( \|\partial \Lcal / \partial \Wcal_j^{(1)}\|_1 \). Reactivation occurs when
    \begin{displaymath}
        M\left\|\frac{\partial \Lcal}{\partial \Wcal_j^{(1)}}\right\|_1 > (\delta + \epsilon)\lambda_k,
    \end{displaymath}
    which can be satisfied for any \( \epsilon > 0 \) in problem instances where mode \( j \) is informative through the network path.
\end{proof}

Without input masking, \( \partial \Lcal / \partial \Wcal_j^{(1)} \neq \mathbf{0} \) even when \( \omega_j = 0 \). This produces a nonzero \( \ot{\Wcal}_j^{(1)} \), contributing the term \( M\|\ot{\Wcal}_j^{(1)}\|_1 \) to the Hier-Prox threshold. If this term is large enough, the threshold is exceeded and the mode reactivates.

\subsubsection{Failure with \texorpdfstring{$\ell_1$}{L1}-Penalty Alone}

\begin{corollary}\label{cor:l1_failure}
    Consider an architecture with \( \ell_1 \)-penalty on \( \omegavec \) but without the Hierarchical~\Cref{ass:hier}. Monotonic mode elimination is not guaranteed, even with input masking and~\Cref{ass:lipschitz,ass:margin}.
\end{corollary}

\begin{proof}
    Without the hierarchical constraint, the proximal update for \( \omega_j \) is soft-thresholding: \( \omega_j^+ = \mathcal{S}_{\alpha\lambda}(\ot{\omega}_j) \), where \( \mathcal{S}_\tau(x) = \mathrm{sign}(x)\max(|x| - \tau, 0) \)~\cite{parikh2014proximal}.
    
    Consider the iteration at which \( \omega_j \) first reaches zero while \( \Wcal_j^{(1)} \) may be nonzero. Suppose at iteration \( t \), we have \( \omega_j^{(t)} = 0 \) but \( \Wcal_j^{(1)(t)} \neq \mathbf{0} \). By~\Cref{fact:jacobian_column}, \( \Wcal_j^{(1)} \neq \mathbf{0} \) implies \( \Jmat_\hnn(\zetavec)\evec_j \neq \mathbf{0} \), hence \( G_j^{\mathrm{net}} \neq 0 \) by~\eqref{eqn:Gnet}.
    
    The preproximal value is
    \begin{displaymath}
        \ot{\omega}_j = -\alpha(G_j^{\mathrm{skip}} + G_j^{\mathrm{net}}).
    \end{displaymath}
    Soft-thresholding gives \( \omega_j^{(t+1)} = 0 \) only if \( |G_j^{\mathrm{skip}} + G_j^{\mathrm{net}}| \leq \lambda \)~\cite{parikh2014proximal}. Even if \( |G_j^{\mathrm{skip}}| \leq (1-\delta)\lambda \) per~\Cref{ass:margin}, the term \( G_j^{\mathrm{net}} \) can cause the sum to exceed \( \lambda \), yielding
    \begin{displaymath}
        \omega_j^{(t+1)} = \mathcal{S}_{\alpha\lambda}(-\alpha(G_j^{\mathrm{skip}} + G_j^{\mathrm{net}})) \neq 0,
    \end{displaymath}
    and mode \( j \) is reactivated.
\end{proof}

The mechanism underlying~\Cref{cor:l1_failure} is the dependence of \( \Jmat_\hnn(\zetavec)\evec_j \) on \( \Wcal_j^{(1)} \) established in~\Cref{fact:jacobian_column}. Even though input masking ensures the \gls{nn} \emph{output} does not depend on \( \Wcal_j^{(1)} \) when \( \omega_j = 0 \), the \emph{sensitivity} \( \Jmat_\hnn \evec_j \) does depend on \( \Wcal_j^{(1)} \). This sensitivity appears in \( G_j^{\mathrm{net}} \) and hence in \( \partial \Lcal / \partial \omega_j \).

% \subsection{Summary of design choice}

% Monotonic mode elimination requires:
% \begin{enumerate}
%     \item \textbf{Input masking} (\Cref{lem:gradient_severance}): Ensures \( \partial \Lcal / \partial \Wcal_j^{(1)} = \mathbf{0} \) when \( \omega_j = 0 \), preventing reactivation through the Hier-Prox threshold.
%     \item \textbf{Hierarchical constraint} (\Cref{lem:weight_null}): Forces \( \Wcal_j^{(1)} = \mathbf{0} \) when \( \omega_j = 0 \), ensuring \( G_j^{\mathrm{net}} = 0 \).
% \end{enumerate}

In summary, neither condition alone suffices: without the hierarchical constraint, \( \Wcal_j^{(1)} \) is not forced to zero (\Cref{cor:l1_failure}); without input masking, gradients are not severed (\Cref{cor:reactivation}). SparseModesNet employs both, achieving the monotonic mode elimination of~\Cref{thm:sup:monotonic}.



